Black-box Coreset Variational Inference

Recent advances in coreset methods have shown that a selection of representative datapoints can replace massive volumes of data for Bayesian inference, preserving the relevant statistical information and significantly accelerating subsequent downstream tasks. Existing variational coreset constructions rely on either selecting subsets of the observed datapoints, or jointly performing approximate inference and optimizing pseudodata in the observed space akin to inducing points methods in Gaussian Processes. So far, both approaches are limited by complexities in evaluating their objectives for general purpose models, and require generating samples from a typically intractable posterior over the coreset throughout inference and testing. In this work, we present a black-box variational inference framework for coresets that overcomes these constraints and enables principled application of variational coresets to intractable models, such as Bayesian neural networks. We apply our techniques to supervised learning problems, and compare them with existing approaches in the literature for data summarization and inference.

==> neurips22/extended_lr_table.tex <==
\begin{table}[]
\caption{Full trials on webspam dataset}
\resizebox{14cm}{!}{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
    & & \multicolumn{7}{c}{\texttt{webspam}} &  &  \\
    & & \multicolumn{7}{c}{Test accuracies~($\uparrow$)} &   \\
 &  $M$ & 4 & 10 & 20 & 30 & 40 & 50 &  100 & 200  &   \\ \midrule
\multirow{3}{*}{BB PSVI} & &  &  &  & &  &  &  \\
  &   $\bv${$(\star)$}  &   $91.7  \pm 0.3 $  &  $\mathbf{92.2}  \pm 0.1 $  &  $\mathbf{92.3}  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $\mathbf{92.4}  \pm 0.1 $  &  $\mathbf{92.4}  \pm 0.1 $  &  $\mathbf{92.3}  \pm 0.0 $  &  $\mathbf{92.4}  \pm 0.1 $  \\
 &   $\bv${$(\star)$},  $\mathbf{\alpha}$ &    $91.6  \pm 0.4 $  &  $\mathbf{92.2}  \pm 0.2 $  &  $92.1  \pm 0.2 $  &  $\mathbf{92.3}  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $\mathbf{92.3}  \pm 0.1 $  &  $\mathbf{92.4}  \pm 0.1 $  \\
   & $ \bv $ &  $91.8  \pm 0.2 $  &  $\mathbf{92.2}  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $92.1  \pm 0.1 $  &  $92.3  \pm 0.1 $  &  $\mathbf{92.4}  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $92.3  \pm 0.1 $  \\
  &   $\bv$=$\frac{N}{M}\mathbf{1}$ &  $90.3  \pm 2.8 $  &  $90.9  \pm 0.3 $  &  $91.7  \pm 0.7 $  &  $91.7  \pm 0.1 $  &  $91.9  \pm 0.1 $  &  $91.5  \pm 0.5 $  &  $92.2  \pm 0.5 $  &  $92.1  \pm 0.4 $ \\
   &unif. IW, $(\star)$  &  $\mathbf{91.9}  \pm 0.2 $  &  $92.1  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $92.3  \pm 0.1 $  &  $\mathbf{92.4}  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $92.3  \pm 0.1 $ \\
    &   w/o IW, $(\star)$ &   $87.6  \pm 3.4 $  &  $90.1  \pm 0.6 $  &  $91.5  \pm 0.1 $  &  $91.7  \pm 0.3 $  &  $92.0  \pm 0.1 $  &  $92.2  \pm 0.1 $  &  $92.3  \pm 0.1 $  &  $\mathbf{92.4}  \pm 0.2 $    \\
     &    $\bv$=$\mathbf{1}$ &   $61.6  \pm 1.0 $  &  $61.1  \pm 1.8 $  &  $61.2  \pm 2.6 $  &  $61.2  \pm 2.6 $  &  $61.2  \pm 4.7 $  &  $61.2  \pm 2.7 $  &  $61.2  \pm 2.2 $  &  $61.2  \pm 1.9 $  \\
\multirow{1}{*}{Sparse BBVI } 
& Batch &   $68.6  \pm 0.9 $  &  $80.1  \pm 0.9 $  &  $84.5  \pm 1.1 $  &  $86.0  \pm 0.4 $  &  $86.9  \pm 0.2 $  &  $87.2  \pm 0.3 $  &  $88.9  \pm 0.4 $  &  $90.3  \pm 0.0 $    \\
& Incr. &   $33.3  \pm 11.8 $  &  $61.2  \pm 0.6 $ &  $61.2  \pm 0.6 $ & $64.0  \pm 2.3 $ & $65.6  \pm 1.2 $ &   $65.6  \pm 1.2 $ & $74.9  \pm 2.9 $ & $76.6  \pm 1.6 $   \\
\multirow{1}{*}{PSVI~\citep{psvi20}} & &  $79.4  \pm 2.3 $  &  $83.9  \pm 0.7 $  &  $87.5  \pm 0.9 $  &  $88.3  \pm 0.3 $  &  $88.8  \pm 0.4 $  &  $89.2  \pm 0.2 $  &  $90.3  \pm 0.3 $  &  $89.8  \pm 0.2 $ \\
\multirow{1}{*}{Subset Laplace} & &  $61.2  \pm 0.1 $  &  $65.6  \pm 0.0 $  &  $65.4  \pm 0.0 $  &  $67.2  \pm 0.0 $  &  $66.6  \pm 0.0 $  &  $67.6  \pm 0.0 $  &  $67.0  \pm 0.0 $  &  $66.5  \pm 0.0 $   \\
 \multirow{1}{*}{Rand. Coreset} & &  $68.7  \pm 2.0 $  &  $71.3  \pm 2.9 $  &  $76.7  \pm 1.1 $  &  $80.7  \pm 0.8 $  &  $83.6  \pm 1.2 $  &  $80.9  \pm 1.5 $  &  $86.3  \pm 0.6 $  &  $87.1  \pm 0.6 $   \\
 \multirow{1}{*}{Full MFVI} & & & & & & & & & $\mathbf{92.7}  \pm 0.0 $ 
\\ \bottomrule
\end{tabular}  
}
\resizebox{14cm}{!}{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
    & & \multicolumn{7}{c}{\texttt{webspam}} &  &  \\
    & & \multicolumn{7}{c}{Test negative log. likelihood~($\downarrow$)} &   \\
 &  $M$ & 4 & 10 & 20 & 30 & 40 & 50 &  100 & 200  &   \\ \midrule
\multirow{3}{*}{BB PSVI} & &  &  &  & &  &  &  \\
  &   $\bv${$(\star)$}  & $23.4  \pm 1.2 $  &  $21.7  \pm 0.3 $  &  $21.4  \pm 0.2 $  &  $22.2  \pm 0.2 $  &  $21.9  \pm 0.2 $  &  $21.3  \pm 0.1 $  &  $21.2  \pm 0.2 $  &  $20.6  \pm 0.2 $  \\
 &   $\bv${$(\star)$},  $\mathbf{\alpha}$ &  $23.8  \pm 1.6 $  &  $22.1  \pm 0.5 $  &  $21.7  \pm 0.1 $  &  $21.4  \pm 0.1 $  &  $21.6  \pm 0.2 $  &  $21.4  \pm 0.2 $  &  $21.0  \pm 0.0 $  &  $20.6  \pm 0.0 $ \\
   & $ \bv $ &  $24.0  \pm 1.2 $  &  $21.9  \pm 0.4 $  &  $21.5  \pm 0.2 $  &  $21.9  \pm 0.2 $  &  $21.9  \pm 0.1 $  &  $21.7  \pm 0.1 $  &  $21.6  \pm 0.3 $  &  $21.5  \pm 0.1 $ \\
  &   $\bv$=$\frac{N}{M}\mathbf{1}$ &  $67.7  \pm 10.6 $  &  $40.8  \pm 0.8 $  &  $53.3  \pm 6.8 $  &  $59.2  \pm 7.1 $  &  $57.7  \pm 10.9 $  &  $54.4  \pm 9.2 $  &  $25.9  \pm 0.1 $  &  $25.9  \pm 0.1 $ \\
   &unif. IW, $(\star)$  & $\mathbf{22.5}  \pm 0.8 $  &  $\mathbf{21.2}  \pm 0.2 $  &  $\mathbf{21.0}  \pm 0.2 $  &  $\mathbf{21.0}  \pm 0.2 $  &  $\mathbf{20.8}  \pm 0.1 $  &  $\mathbf{20.6}  \pm 0.1 $  &  $\mathbf{20.8}  \pm 0.1 $  &  $\mathbf{20.5}  \pm 0.0 $ \\
    &   w/o IW, $(\star)$ & $49.6  \pm 7.7 $  &  $29.8  \pm 2.1 $  &  $23.9  \pm 0.6 $  &  $22.8  \pm 1.0 $  &  $21.8  \pm 0.4 $  &  $22.0  \pm 0.3 $  &  $21.2  \pm 0.3 $  &  $20.8  \pm 0.3 $ \\
    &    $\bv$=$\mathbf{1}$ & $69.5  \pm 0.6 $  &  $69.4  \pm 3.2 $  &  $73.5  \pm 2.1 $  &  $71.3  \pm 5.3 $  &  $78.4  \pm 4.9 $  &  $71.4  \pm 5.5 $  &  $70.4  \pm 4.7 $  &  $71.1  \pm 5.5 $   \\
\multirow{1}{*}{Sparse BBVI } 
& Batch &     $97.8  \pm 6.3 $  &  $65.0  \pm 8.6 $  &  $43.4  \pm 1.3 $  &  $39.2  \pm 0.5 $  &  $39.1  \pm 1.6 $  &  $36.9  \pm 0.6 $  &  $35.9  \pm 1.2 $  &  $32.1  \pm 1.0 $ \\
& Incr. &    $69.7  \pm 0.5 $ & $66.8  \pm 4.2 $ & $66.8  \pm 4.2 $ & $60.3  \pm 7.0 $ & $65.8  \pm 1.6 $ & $65.8  \pm 1.6 $ & $60.4  \pm 3.0 $ & $50.8  \pm 1.2 $   \\
\multirow{1}{*}{PSVI~\citep{psvi20}} &  & $46.4  \pm 3.1 $  &  $32.5  \pm 3.1 $  &  $57.4  \pm 4.8 $  &  $42.8  \pm 8.4 $  &  $51.2  \pm 16.9 $  &  $26.1  \pm 8.4 $  &  $26.0  \pm 0.1 $  &  $26.0  \pm 0.0 $  \\
\multirow{1}{*}{Subset Laplace} &  & $67.0  \pm 0.8 $  &  $62.0  \pm 0.0 $  &  $59.9  \pm 0.0 $  &  $57.7  \pm 0.0 $  &  $58.1  \pm 0.0 $  &  $57.3  \pm 0.0 $  &  $57.7  \pm 0.0 $  &  $58.7  \pm 0.0 $  \\
 \multirow{1}{*}{Rand. Coreset} & & $184.4  \pm 48.7 $  &  $175.1  \pm 25.3 $  &  $124.8  \pm 8.6 $  &  $96.6  \pm 12.0 $  &  $76.9  \pm 15.5 $  &  $129.3  \pm 15.5 $  &  $83.1  \pm 5.8 $  &  $86.5  \pm 3.8 $   \\
 \multirow{1}{*}{Full MFVI} & & & & & & & & & $\mathbf{19.8}  \pm 0.0 $
\\ \bottomrule
\end{tabular}  
}
\label{tab:webspam-lr-comparison}
\end{table}


\begin{table}[]
\caption{Full trials on phishing dataset}
\resizebox{14cm}{!}{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
    & & \multicolumn{7}{c}{\texttt{phishing}} &  &  \\
    & & \multicolumn{7}{c}{Test accuracies~($\downarrow$)} &   \\
 &  $M$ & 4 & 10 & 20 & 30 & 40 & 50 &  100 & 200  &   \\ \midrule
\multirow{3}{*}{BB PSVI} & &  &  &  & &  &  &  \\
  &   $\bv${$(\star)$} &  $82.0  \pm 3.6 $  &  $90.1  \pm 0.5 $  &  $90.5  \pm 1.1 $  &  $\mathbf{91.0}  \pm 1.0 $  &  $\mathbf{91.2}  \pm 1.0 $  &  $\mathbf{90.6}  \pm 0.8 $  &  $90.4  \pm 0.0 $  &  $90.3  \pm 0.0 $   \\
 &   $\bv${$(\star)$},  $\mathbf{\alpha}$ &  $82.3  \pm 3.7 $  &  $90.7  \pm 0.5 $  &  $91.1  \pm 1.2 $  &  $90.7  \pm 0.8 $  &  $90.7  \pm 0.9 $  &  $\mathbf{90.6}  \pm 0.2 $  &  $90.4  \pm 0.0 $  &  $90.4  \pm 0.0 $  \\
   & $ \bv $ & $ 81.3  \pm 2.7 $  &  $90.3  \pm 0.8 $  &  $90.0  \pm 1.0 $  &  $88.8  \pm 0.9 $  &  $89.8  \pm 0.2 $  &  $90.1  \pm 0.4 $  &  $90.3  \pm 0.1 $  &  $90.2  \pm 0.4 $  \\
  &   $\bv$=$\frac{N}{M}\mathbf{1}$ & $79.5  \pm 2.8 $  &  $90.2  \pm 0.3 $  &  $88.8  \pm 0.7 $  &  $90.0  \pm 0.3 $  &  $88.9  \pm 0.7 $  &  $89.8  \pm 0.5 $  &  $\mathbf{90.5}  \pm 0.0 $  &  $90.4  \pm 0.1 $  \\
   &unif. IW, $(\star)$  &  $\mathbf{85.7}  \pm 3.5 $  &  $\mathbf{90.8}  \pm 1.0 $  &  $\mathbf{91.3}  \pm 1.7 $  &  $90.7  \pm 1.3 $  &  $90.6  \pm 0.9 $  &  $90.4  \pm 0.1 $  &  $90.4  \pm 0.0 $  &  $90.4  \pm 0.0 $  \\
    &   w/o IW, $(\star)$ & $80.0  \pm 0.5 $  &  $90.1  \pm 1.4 $  &  $90.4  \pm 1.2 $  &  $90.4  \pm 1.5 $  &  $89.2  \pm 1.2 $  &  $88.0  \pm 1.2 $  &  $90.4  \pm 0.2 $  &  $90.3  \pm 0.2 $    \\
    &    $\bv$=$\mathbf{1}$ &   $80.4  \pm 12.7 $  &  $85.8  \pm 10.4 $  &  $85.2  \pm 11.1 $  &  $86.3  \pm 11.2 $  &  $86.3  \pm 11.1 $  &  $86.7  \pm 11.3 $  &  $87.3  \pm 11.5 $  &  $82.2  \pm 10.2 $ 
   \\
\multirow{1}{*}{Sparse BBVI } 
& Batch &   $70.0  \pm 7.5 $  &  $87.6  \pm 0.8 $  &  $88.1  \pm 0.4 $  &  $88.8  \pm 1.0 $  &  $90.7  \pm 0.3 $  &  $90.1  \pm 0.3 $  &  $90.2  \pm 1.2 $  &  $90.3  \pm 0.0 $   \\
& Incr. &  $45.8  \pm 4.2 $ & $88.8  \pm 2.1 $ & $88.8  \pm 2.1 $ &  $83.4  \pm 1.0 $ & $82.4  \pm 2.1 $  & $82.4  \pm 2.1 $  & $88.6  \pm 2.1 $ &  $\mathbf{90.8}  \pm 2.9 $ \\
\multirow{1}{*}{PSVI~\citep{psvi20}} & & $80.4  \pm 2.1 $  &  $88.3  \pm 1.7 $  &  $87.9  \pm 1.7 $  &  $89.4  \pm 0.4 $  &  $89.0  \pm 0.9 $  &  $90.1  \pm 0.3 $  &  $90.1  \pm 0.1 $  &  $90.2  \pm 0.0 $  \\
\multirow{1}{*}{Subset Laplace} &  & $40.1  \pm 5.5 $  &  $69.1  \pm 0.0 $  &  $75.8  \pm 0.0 $  &  $75.7  \pm 0.0 $  &  $77.6  \pm 0.0 $  &  $78.6  \pm 0.0 $  &  $79.6  \pm 0.0 $  &   $79.7  \pm 0.0 $  \\
 \multirow{1}{*}{Rand. Coreset} & & $74.8  \pm 3.9 $  &  $81.4  \pm 2.7 $  &  $87.6  \pm 0.6 $  &  $80.6  \pm 2.4 $  &  $86.1  \pm 3.8 $  &  $86.1  \pm 2.9 $  &  $84.4  \pm 1.7 $  &  $89.5  \pm 0.9 $    \\
 \multirow{1}{*}{Full MFVI} & & & & & & & & & $\mathbf{90.4}  \pm 0.0 $ 
\\ \bottomrule
\end{tabular}  
}
\resizebox{14cm}{!}{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
    & & \multicolumn{7}{c}{\texttt{phishing}} &  &  \\
    & & \multicolumn{7}{c}{Test negative log. likelihood~($\downarrow$)} &   \\
 &  $M$ & 4 & 10 & 20 & 30 & 40 & 50 &  100 & 200  &   \\ \midrule
\multirow{3}{*}{BB PSVI} & &  &  &  & &  &  &  \\
  &   $\bv${$(\star)$}  & $51.5  \pm 14.1 $  &  $36.1  \pm 0.8 $  &  $42.2  \pm 1.0 $  &  $35.6  \pm 2.2 $  &  $34.8  \pm 3.8 $  &  $35.1  \pm 3.1 $  &  $26.0  \pm 0.1 $  &  $26.0  \pm 0.1 $  \\
 &   $\bv${$(\star)$},  $\mathbf{\alpha}$ &  $47.5  \pm 14.6 $  &  $33.6  \pm 0.6 $  &  $35.5  \pm 1.9 $  &  $33.7  \pm 2.3 $  &  $34.2  \pm 3.1 $  &  $31.9  \pm 1.9 $  &  $\mathbf{25.9}  \pm 0.1 $  &  ${25.9}  \pm 0.1 $   \\
   & $ \bv $ & $60.4  \pm 9.6 $  &  $40.3  \pm 2.1 $  &  $49.8  \pm 1.3 $  &  $49.7  \pm 6.5 $  &  $48.9  \pm 6.2 $  &  $49.6  \pm 6.6 $  &  $26.0  \pm 0.1 $  &  $26.3  \pm 0.7 $  \\
  &   $\bv$=$\frac{N}{M}\mathbf{1}$ &  $67.7  \pm 10.6 $  &  $40.8  \pm 0.8 $  &  $53.3  \pm 6.8 $  &  $59.2  \pm 7.1 $  &  $57.7  \pm 10.9 $  &  $54.4  \pm 9.2 $  &  $\mathbf{25.9}  \pm 0.1 $  &  ${25.9}  \pm 0.1 $  \\
   &unif. IW, $(\star)$  & $\mathbf{39.2}  \pm 12.0 $  &  $\mathbf{31.8}  \pm 1.8 $  &  $37.0  \pm 2.7 $  &  $\mathbf{32.9}  \pm 2.4 $  &  $\mathbf{31.3}  \pm 2.7 $  &  $29.4  \pm 1.3 $  &  $\mathbf{25.9}  \pm 0.1 $  &  $26.0  \pm 0.1 $  \\
    &   w/o IW, $(\star)$ &  $75.5  \pm 5.6 $  &  $43.8  \pm 5.5 $  &  $43.4  \pm 5.1 $  &  $36.1  \pm 6.9 $  &  $35.8  \pm 6.3 $  &  $36.2  \pm 6.4 $  &  $26.9  \pm 0.5 $  &  $26.9  \pm 0.4 $  \\
    &    $\bv$=$\mathbf{1}$ &    $\mathbf{39.2}  \pm 37.8 $  &  $37.5  \pm 24.4 $  &  $36.9  \pm 25.9 $  &  $36.5  \pm 24.6 $  &  $34.7  \pm 23.6 $  &  $36.0  \pm 24.2 $  &  $38.3  \pm 24.8 $  &  $41.1  \pm 24.1 $   \\
\multirow{1}{*}{Sparse BBVI } 
& Batch &  $81.8  \pm 21.3 $  &  $40.2  \pm 2.9 $  &  $43.6  \pm 3.1 $  &  $43.1  \pm 3.3 $  &  $35.2  \pm 0.9 $  &  $34.4  \pm 2.6 $  &  $\mathbf{25.9}  \pm 2.1 $  &  ${25.9}  \pm 0.1 $    \\
& Incr. &  $73.3  \pm 2.7 $ & $33.6  \pm 3.6 $ & $\mathbf{33.6}  \pm 3.6 $ & $38.0  \pm 1.9 $ &  $38.0  \pm 1.9 $  & $38.0  \pm 1.9 $ & $30.8  \pm 3.7$  & $\mathbf{25.3}  \pm 4.9$ \\
\multirow{1}{*}{PSVI~\citep{psvi20}} & &  $46.4  \pm 3.1 $  &  $32.5  \pm 3.1 $  &  $57.4  \pm 4.8 $  &  $42.8  \pm 8.4 $  &  $51.2  \pm 16.9 $  &  $\mathbf{26.1}  \pm 8.4 $  &  $26.0  \pm 0.1 $  &  $26.0  \pm 0.0 $ \\
\multirow{1}{*}{Subset Laplace} &  &  $75.3  \pm 1.3 $  &  $66.5  \pm 0.0 $  &  $56.2  \pm 0.0 $  &  $54.7  \pm 0.0 $  &  $51.1  \pm 0.0 $  &  $49.8  \pm 0.0 $  &  $48.8  \pm 0.0 $  &  $47.2  \pm 0.0 $  &   \\
 \multirow{1}{*}{Rand. Coreset} & &  $113.2  \pm 19.3 $  &  $122.0  \pm 13.4 $  &  $82.5  \pm 2.7 $  &  $159.2  \pm 28.5 $  &  $156.0  \pm 53.0 $  &  $188.7  \pm 59.0 $  &  $47.6  \pm 3.4 $  &  $30.2  \pm 1.0 $ 
    \\
 \multirow{1}{*}{Full MFVI} & & & & & & & & & ${26.1}  \pm 0.1 $
\\ \bottomrule
\end{tabular}  
}
\label{tab:phishing-lr-comparison}
\end{table}


\begin{table}[]
\caption{Full trials on adult dataset}
\resizebox{15cm}{!}{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
    & & \multicolumn{7}{c}{\texttt{adult}} &  &  \\
    & & \multicolumn{7}{c}{Test accuracies~($\uparrow$)} &   \\
 &  $M$ & 4 & 10 & 20 & 30 & 40 & 50 &  100 & 200  &   \\ \midrule
\multirow{3}{*}{BB PSVI} & &  &  &  & &  &  &  \\
  &   $\bv${$(\star)$}  &  $81.7  \pm 3.5 $  &  $82.2  \pm 0.9 $  &  $82.1  \pm 0.3 $  &  $83.3  \pm 0.3 $  &  $\mathbf{83.5}  \pm 0.2 $  &  $83.5  \pm 0.0 $  &  $83.5  \pm 0.0 $  &  $\mathbf{83.5}  \pm 0.0 $  \\
 &   $\bv${$(\star)$},  $\mathbf{\alpha}$ &  $81.7  \pm 3.4 $  &  $\mathbf{82.6}  \pm 0.9 $  &  $83.2  \pm 0.6 $  &  $83.3  \pm 0.3 $  &  $\mathbf{83.5}  \pm 0.0 $  &  $83.5  \pm 0.1 $  &  $\mathbf{83.6}  \pm 0.0 $  &  $\mathbf{83.5}  \pm 0.0 $   \\
   & $ \bv $ & $81.6  \pm 1.0 $  &  $82.4  \pm 0.4 $  &  $\mathbf{83.3}  \pm 0.4 $  &  $83.0  \pm 0.4 $  &  $\mathbf{83.5}  \pm 0.0 $  &  $\mathbf{83.6}  \pm 0.0 $  &  $83.5  \pm 0.0 $  &  $\mathbf{83.5}  \pm 0.0 $  \\
  &   $\bv$=$\frac{N}{M}\mathbf{1}$ & $80.1  \pm 5.1 $  &  $81.0  \pm 0.4 $  &  $82.0  \pm 0.1 $  &  $\mathbf{83.5}  \pm 0.3 $  &  $\mathbf{83.5}  \pm 0.1 $  &  $83.5  \pm 0.0 $  &  $83.5  \pm 0.5 $  &  $\mathbf{83.5}  \pm 0.0 $   \\
   &unif. IW, $(\star)$  &  $\mathbf{82.2}  \pm 3.3 $  &  $82.1  \pm 0.8 $  &  $83.2  \pm 0.4 $  &  $83.1  \pm 0.1 $  &  $\mathbf{83.5}  \pm 0.1 $  &  $\mathbf{83.6}  \pm 0.0 $  &  $83.5  \pm 0.0 $  &  $\mathbf{83.5}  \pm 0.0 $   \\
    &   w/o IW, $(\star)$ &  $77.2  \pm 4.7 $  &  $77.8  \pm 1.5 $  &  $82.7  \pm 0.8 $  &  $\mathbf{83.5}  \pm 0.9 $  &  $\mathbf{83.5}  \pm 0.0 $  &  $83.5  \pm 0.4 $  &  $83.5  \pm 0.1 $  &  $\mathbf{83.5}  \pm 0.0 $  \\
    &    $\bv$=$\mathbf{1}$ &   $73.2  \pm 3.2 $  &  $75.0  \pm 3.7 $  &  $75.2  \pm 1.8 $  &  $75.2  \pm 2.3 $  &  $75.1  \pm 1.6 $  &  $75.1  \pm 1.3 $  &  $75.8  \pm 1.2 $  &  $75.3  \pm 1.3 $  \\
\multirow{1}{*}{Sparse BBVI } 
& Batch &    $77.5  \pm 4.6 $  &  $78.1  \pm 1.1 $  &  $80.2  \pm 0.8 $  &  $81.9  \pm 0.5 $  &  $82.6  \pm 0.4 $  &  $82.5  \pm 0.9 $  &  $83.5  \pm 0.7 $  &  $\mathbf{83.5}  \pm 0.0 $  \\
& Incr. &   $44.8  \pm 6.1 $  &  $81.3  \pm 1.0 $  &  $81.3  \pm 1.0 $ & $80.0  \pm 0.8 $ & $79.0  \pm 1.7 $ & $79.0  \pm 1.7 $ & $81.7  \pm 0.9 $ &  $83.1  \pm 0.1 $ \\
\multirow{1}{*}{PSVI~\citep{psvi20}} & & $80.1  \pm 1.5 $  &  $82.5  \pm 0.4 $  &  $81.8  \pm 0.5 $  &  $83.3  \pm 0.4 $  &  $83.5  \pm 0.0 $  &  $83.4  \pm 0.4 $  &  $83.5  \pm 0.0 $  &  $\mathbf{83.5}  \pm 0.0 $   \\
\multirow{1}{*}{Subset Laplace} & &  $44.9  \pm 0.9 $  &  $75.3  \pm 0.0 $  &  $76.5  \pm 0.0 $  &  $77.2  \pm 0.0 $  &  $78.2  \pm 0.0 $  &  $78.7  \pm 0.0 $  &  $79.3  \pm 0.0 $  &  $79.8  \pm 0.0 $  &    \\
 \multirow{1}{*}{Rand. Coreset} &  &  $74.2  \pm 8.0 $  &  $75.9  \pm 1.1 $  &  $78.9  \pm 2.4 $  &  $77.5  \pm 1.0 $  &  $76.2  \pm 0.3 $  &  $77.3  \pm 1.1 $  &  $79.5  \pm 0.5 $  &  $82.1  \pm 0.3 $   \\
 \multirow{1}{*}{Full MFVI} & & & & & & & & & $\mathbf{83.5}  \pm 0.0 $
\\ \bottomrule
\end{tabular}  
}
\resizebox{15cm}{!}{
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
    & & \multicolumn{7}{c}{\texttt{adult}} &  &  \\
    & & \multicolumn{7}{c}{Test negative log. likelihood~($\downarrow$)} &   \\
 &  $M$ & 4 & 10 & 20 & 30 & 40 & 50 &  100 & 200  &   \\ \midrule
\multirow{3}{*}{BB PSVI} & &  &  &  & &  &  &  \\
  &   $\bv${$(\star)$} & $52.2  \pm 14.3 $  &  $55.0  \pm 6.3 $  &  $48.5  \pm 1.2 $  &  $34.1  \pm 4.9 $  &  $\mathbf{33.9}  \pm 0.3 $  &  $34.0  \pm 0.0 $  &  $\mathbf{33.9}  \pm 0.0 $  &  $\mathbf{33.9}  \pm 0.0 $    \\
 &   $\bv${$(\star)$},  $\mathbf{\alpha}$ & $49.2  \pm 10.0 $  &  $50.2  \pm 3.2 $  &  $47.8  \pm 3.9 $  &  $44.2  \pm 3.0 $  &  $34.0  \pm 0.0 $  &  $\mathbf{33.9}  \pm 0.1 $  &  $\mathbf{33.9}  \pm 0.0 $  &  $\mathbf{33.9}  \pm 0.0 $   \\
   & $ \bv $ & $63.8  \pm 23.4 $  &  $78.0  \pm 6.2 $  &  $70.0  \pm 13.4 $  &  $40.2  \pm 3.9 $  &  $34.0  \pm 0.1 $  &  $\mathbf{33.9}  \pm 0.0 $  &  $34.0  \pm 0.1 $  &  $\mathbf{33.9}  \pm 0.0 $  \\
  &   $\bv$=$\frac{N}{M}\mathbf{1}$ & $70.3  \pm 28.4 $  &  $79.5  \pm 14.5 $  &  $60.4  \pm 4.5 $  &  $\mathbf{34.0}  \pm 9.5 $  &  $\mathbf{33.9}  \pm 0.1 $  &  $\mathbf{33.9}  \pm 0.0 $  &  $\mathbf{33.9}  \pm 1.4 $  &  $\mathbf{33.9}  \pm 0.0 $   \\
   &unif. IW, $(\star)$  &  $\mathbf{45.7}  \pm 14.6 $  &  $48.1  \pm 2.2 $  &  $45.5  \pm 3.2 $  &  $34.5  \pm 2.7 $  &  $\mathbf{33.9}  \pm 0.1 $  &  $\mathbf{33.9}  \pm 0.0 $  &  $\mathbf{33.9}  \pm 0.1 $  &  $\mathbf{33.9}  \pm 0.0 $   \\
    &   w/o IW, $(\star)$ & $96.4  \pm 23.7 $  &  $74.9  \pm 10.2 $  &  $44.7  \pm 11.2 $  &  $34.5  \pm 6.8 $  &  $34.2  \pm 0.1 $  &  $34.1  \pm 3.3 $  &  $34.0  \pm 0.3 $  &  $34.0  \pm 0.0 $  \\
    &    $\bv$=$\mathbf{1}$ &   $54.5  \pm 4.7 $  &  $57.7  \pm 7.1 $  &  $58.3  \pm 4.7 $  &  $56.7  \pm 5.5 $  &  $53.1  \pm 3.6 $  &  $53.0  \pm 2.6 $  &  $49.4  \pm 3.0 $  &  $51.1  \pm 3.1 $   \\
\multirow{1}{*}{Sparse BBVI } 
& Batch &   $73.8  \pm 17.6 $  &  $70.8  \pm 4.4 $  &  $62.2  \pm 4.8 $  &  $57.4  \pm 9.2 $  &  $48.3  \pm 1.6 $  &  $49.1  \pm 4.2 $  &  $\mathbf{33.9}  \pm 10.2 $  &  $\mathbf{33.9}  \pm 0.0 $    \\
& Incr. &  $72.2  \pm 2.0 $  &  $41.5  \pm 0.6 $    &  $\mathbf{41.5}  \pm 0.6 $   & $41.9  \pm 1.8 $  & $41.6  \pm 2.0 $ & $41.6  \pm 2.0 $  & $39.1  \pm 1.8 $  & $38.1  \pm 1.0 $   \\
\multirow{1}{*}{PSVI~\citep{psvi20}} & & $46.6  \pm 2.2 $  &  $\mathbf{40.7}  \pm 2.4 $  &  $44.7  \pm 10.2 $  &  $34.6  \pm 8.8 $  &  $34.0  \pm 0.1 $  &  $34.0  \pm 5.4 $  &  $34.0  \pm 0.0 $  &  $34.0  \pm 0.0 $  \\
\multirow{1}{*}{Subset Laplace} &  &  $75.3  \pm 1.3 $  &  $66.5  \pm 0.0 $  &  $56.2  \pm 0.0 $  &  $54.7  \pm 0.0 $  &  $51.1  \pm 0.0 $  &  $49.8  \pm 0.0 $  &  $48.8  \pm 0.0 $  &  $47.2  \pm 0.0 $  &   \\
 \multirow{1}{*}{Rand. Coreset} & &   $324.5  \pm 52.3 $  &  $251.4  \pm 32.1 $  &  $248.7  \pm 36.6 $  &  $296.4  \pm 10.3 $  &  $178.5  \pm 39.5 $  &  $66.6  \pm 19.5 $  &  $51.8  \pm 6.7 $  &  $39.2  \pm 1.5 $      \\
 \multirow{1}{*}{Full MFVI} & & & & & & & & & $\mathbf{33.9}  \pm 0.0 $ 
\\ \bottomrule
\end{tabular}  
}
\label{tab:adult-lr-comparison}
\end{table}
